The TV is Smart and Full of Trackers: Towards Understanding the Smart TV Advertising and Tracking Ecosystem

Motivated by the growing popularity of smart TVs, we present a large-scale measurement study of smart TVs by collecting and analyzing their network traffic from two different vantage points. First, we analyze aggregate network traffic of smart TVs in-the-wild, collected from residential gateways of tens of homes and several different smart TV platforms, including Apple, Samsung, Roku, and Chromecast. In addition to accessing video streaming and cloud services, we find that smart TVs frequently connect to well-known as well as platform-specific advertising and tracking services (ATS). Second, we instrument Roku and Amazon Fire TV, two popular smart TV platforms, by setting up a controlled testbed to systematically exercise the top-1000 apps on each platform, and analyze their network traffic at the granularity of the individual apps. We again find that smart TV apps connect to a wide range of ATS, and that the key players of the ATS ecosystems of the two platforms are different from each other and from that of the mobile platform. Third, we evaluate the (in)effectiveness of state-of-the-art DNS-based blocklists in filtering advertising and tracking traffic for smart TVs. We find that personally identifiable information (PII) is exfiltrated to platform-related Internet endpoints and third parties, and that blocklists are generally better at preventing exposure of PII to third parties than to platform-related endpoints. Our work demonstrates the segmentation of the smart TV ATS ecosystem across platforms and its differences from the mobile ATS ecosystem, thus motivating the need for designing privacy-enhancing tools specifically for each smart TV platform.

==> analysis.tex <==
\section{Evaluating Block Lists }
\label{sect:filter-list-analysis}



%Our goal is to understand the effectiveness of readily available privacy-preserving tools when applied to smart TVs.
%We apply four popular filter lists to the datasets described in Sections~\ref{sec:in-the-wild} and~\ref{sec:popular-app-testing}.
%In Sec.~\ref{sec:labelling-analysis}, we compare the four filter lists' coverage and show that hostnames that are contacted by multiple apps---referred to as \emph{shared hostnames}---are more likely to be \blue{(labeled as)} \ats{} endpoints.
%Section~\ref{sec:piis-list-analysis} examines the filter lists' ability to prevent exposure of Personally Identifiable Information (\pii{})
%In Sec.~\ref{sec:fneg-analysis}, we investigate the shared hostnames that are not blocked by the filter lists to uncover false negatives.
%Finally, in Sec~\ref{sec:fpos-analysis}, we apply each of the four filter lists while manually interacting with ten apps from the \roku{} and \firetv{} ecosystems to determine if false positives cause app breakage.


\input{analysis_labelling}
\input{analysis_pii}

\input{analysis_fpos}
\input{analysis_fneg}


\begin{comment}
\begin{table}[]
	\begin{tabular}{@{}l|llll@{}}
		\multicolumn{1}{c|}{FireTV} & \multicolumn{4}{c}{\% of Blocked Flows (no Amazon, no IPs)} \\
		\textbf{Rank Interval}& \textbf{MoAAB} & \textbf{Pi-Hole} & \textbf{Firebog} & \textbf{StopAd} \\ \toprule
		{[}1, 200) &  36\% &  41\% &  46\% & 10\% \\
		{[}200, 400) & 36\% & 40\% & 43\% &  11\% \\
		{[}400, 600) & 44\% & 44\% &  50\% &  14\% \\
		{[}600, 800) & 22\% & 22\% &  27\% &  8\% \\
		{[}800, 1K) & 29\% & 31\% &  36\% & 11\%
	\end{tabular}
	\caption{Percentage of Blocked Flows by App Ranking (with no Amazon hosts, no IPs)}
	\label{tab:firetv-app-ranking-blocked-2}
\end{table}

\begin{table}[t!]
	\begin{tabular}{@{}l|llll@{}}
		\multicolumn{1}{c|}{FireTV} & \multicolumn{4}{c}{\% of Blocked Flows (only Amazon+IPs)} \\
		\textbf{Rank Interval}& \textbf{MoAAB} & \textbf{Pi-Hole} & \textbf{Firebog} & \textbf{StopAd} \\ \toprule
		{[}1, 200) &  5\% &  4\% &  4\% & 0\% \\
		{[}200, 400) & 3\% & 3\% & 3\% &  0\% \\
		{[}400, 600) & 5\% & 4\% &  4\% &  0\% \\
		{[}600, 800) & 6\% & 6\% &  6\% &  0\% \\
		{[}800, 1K) & 6\% & 6\% &  6\% & 0\%
	\end{tabular}
	\caption{Percentage of Blocked Flows by App Ranking (with only Amazon hostnames+IPs)}
	\label{tab:firetv-app-ranking-blocked-3}
\end{table}

\end{comment} 

==> analysis_fneg.tex <==

\begin{table}[t!]
	\small
	\begin{tabular}{| c | l | l | r |}
		\cline{2-4} \multicolumn{1}{c|}{} & \textbf{Hostname} & \textbf{Device} & \textbf{\# Apps} \\
		\hline
		\parbox[t]{1mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{In the Wild}}}} & webads.bandsintown.com	& \roku & N/A \\
		& ads-e-darwin.hulustream.com 	& \roku 	& N/A \\
		& track-us.adformnet.akadns.net	& Apple TV	& N/A \\
		& disneyads0-a.akamaihd.net 	& Samsung	& N/A \\
		& advertising.weather.com	& Samsung	& N/A \\
		& tag.adaraanalytics.com	& Vizio	& N/A \\
		\hline
		\parbox[t]{1mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{Testbed}}}} & p.ads.roku.com & \multirow{7}{*}{\roku} & 109 \\
		& ads.ewscloud.com &  & 40 \\
		& collector.vhx.tv &  	& 9 \\
		%attribution.report & \roku 	& \xmark  &   \xmark & \xmark &\xmark  \\
		& trackingrkx.com &  & 4 \\
		& metrics.claspws.tv &  & 4 \\
		%us-east-1-ads.superawesome.tv & \roku 	& \xmark  &   \xmark & \xmark &\xmark \\
		%adtag.primetime.adobe.com & \roku 	& \xmark  &   \xmark & \xmark &\xmark  \\
		& track.sr.roku.com &  & 2 \\
		& router.adstack.tv & & 2 \\
		%static.s3-us-west-1		
		%adplatform-[1].amazonaws.com 		  & \roku 	&\xmark  &   \xmark & \xmark &\xmark   \\
		\hline
		% measurements.s3-external-1
		%kraken-[2].amazonaws.com 	  & \firetv & \xmark  &   \xmark & \xmark &\xmark  \\
		%kinstruments-[2].amazonaws.com  & \firetv & \xmark  &   \xmark & \xmark &\xmark\\
		%venezia-[2].amazonaws.com 	   & \firetv &\xmark  &   \xmark & \xmark &\xmark \\
		\parbox[t]{1mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{Testbed}}}} & firebaseremoteconfig.googleapis.com & \multirow{7}{*}{\firetv} & 17 \\
		& mads.amazon.com & & 8 \\
		& ads.aimitv.com & & 6 \\
		%ads.aimitv.com.s3.amazonaws.com 					   & \firetv & \xmark  &   \xmark & \xmark &\xmark \\
		& analytics.mobitv.com & & 5 \\
		& ad-playlistserver.aws.syncbak.com &  & 5 \\
		& events.brightline.tv &  & 4 \\
		& myhouseofads.firebaseio.com & & 2 \\
		\hline
	\end{tabular}
	\caption{Examples of false negatives for the four filter lists for the hostnames present in the datasets from Sec.~\ref{sec:in-the-wild} and Sec.~\ref{sec:popular-app-testing}.}
	\label{tab:false_negatives}
\end{table}


\descr{False Negatives.}
%In this section, we study the false neagtives
In this section, we examine the four filter lists for false negatives in the context of our smart TV datasets from Sec.~\ref{sec:in-the-wild} and Sec.~\ref{sec:popular-app-testing}.
We define a false negative for a filter list as an \ats{} endpoint that is not covered by that respective list.
In favor of space, we only report on false negatives for the union of the four lists, \ie{}, we examine the set of hostnames that are not labeled as an \ats{} endpoint by \emph{any} of the four lists.

For the \roku{} and \firetv{} datasets from Sec.~\ref{sec:popular-app-testing}, we are able to provide rough estimates of the number of false negatives by counting the number of hostnames that are not blocked by any of the four filter lists, yet still receive any of the PIIs in Table~\ref{tab:pii-firetv-roku}, excluding Account Name and Location.
We exclude the latter two types of PIIs to keep our estimate conservative as these may be sent for legitimate purposes such as to log in or to serve location-based content.
Using this method, we find 38 false negatives in the \roku{} dataset, and 30 false negatives in the \firetv{} dataset.
We stress that these numbers are conservative lower bounds as we only observe for the most basic tracking identifiers that are available through the respective device's settings menu.
More advanced tracking such as device fingerprinting and/or server generated identifiers are not taken into account.
Furthermore, in the case of \roku{}, we are only able to check for PII exposure in the plaintext flows, leaving all PII exposure in the encrypted flows---\blue{which constitute the majority (see Table~X)}---unaccounted for.
A noteworthy mention in these sets of hostnames is \texttt{hotlist.samba.tv}.
Samba TV makes use of Automatic Content Recognition to provide users with content suggestions, but this comes at the cost of targeted advertising that propagates beyond the smart TV to other devices in the home network \cite{sambatv-nyt}.

%As this set of hostnames is too large for manual inspection (\eg, for the \roku{} dataset from Sec.~\ref{sec:popular-app-testing}, this set contains more than 1600 different hostnames), we first filter it, retaining only those hostnames that contain words that are often present in \ats{} hostnames such as ``ad'', ``event'', and ``metric''.
%For the dataset from Sec.~\ref{sec:in-the-wild}, we do not have access to packet payload.
In addition to the PII-based analysis, we also use keyword-based search, as introduced in Sec.~\ref{sec:roku-firetv-all}, on all three datasets to detect potential false negatives.
We then manually inspect the resulting subset of hostnames.
Some of the hostnames in this set are obvious \ats{} endpoints.
For example, for the \roku{} dataset from Sec.~\ref{sec:popular-app-testing}, we see hostnames such as \texttt{p.ads.roku.com} and \texttt{track.sr.roku.com}.
We acknowledge that our string-matching is not perfect as we also see hostnames that appear to be legitimate content delivery endpoints, \eg{}, \texttt{download.inacdn.com} and \texttt{download.ted.com}.
Nevertheless, this simple methodology still manages to identify \blue{(high quality candidate)} false negatives, a small subset of which are summarized in Table~\ref{tab:false_negatives}.
This illustrates that the network traces that can be generated using automation tools such as \rokutool{} and \firetvtool{} may aid in automatically generating high quality candidate rules for filter list currators.
Finally, we note that \blue{[many of]} the false negatives in Table~\ref{tab:false_negatives} are contacted by multiple apps, which further strengthens our belief that these are indeed false negatives as shared hostnames are more likely to be \ats{} endpoints as per our findings in Sec.~\ref{sec:labelling-analysis}.


% \ie, \ats{} endpoints present in our datasets from Sec.~\ref{sec:in-the-wild} and Sec.~\ref{sec:popular-app-testing} which are not covered by the filter lists, but.


%In Sec.~\ref{sect:add-label-to-sect-with-blocking-as-func-of-hostname-sharing} we showed that as the number of apps which contact a given hostname grows, the likelihood that that hostname is an \ats{} endpoint increases (until a point where this tendency plateaus).
%Based on this observation, we hypothesize that false negatives, \ie{}  hostnames which are \ats{} endpoints but are not labeled as such by any of the filter lists, are more likely to be present in the set of hostnames that are only contacted by a single app.

%In Sec.~\ref{sec:add-label-to-sect-with-blocking-as-func-of-hostname-sharing} we showed that as the number of apps which contact a given hostname grows, the likelihood that that hostname is an \ats{} endpoint increases.
%This leaves an interesting question of whether the hostnames that are shared by multiple apps, but not labeled as \ats{} endpoints by any of the filter lists, are indeed true negatives or false negatives.

%We selected


%To gain an understanding of the amount of false negatives


%We investigated this by applying the following procedure.
%For each ecosystem in our \synthdataset, we manually inspected all the hostnames which were contacted by more than one app, but were not blocked by any of the filter lists. Some of these hostnames were obvious CDNs, \eg{} \texttt{amazonchannelstudio-cdn.com} or \texttt{le1.cdn01.net}. Others were clearly \ats{} endpoints -- shown in Table \ref{tab:false_negatives}.
\begin{comment}
\begin{table*}[]
	\small
	\begin{tabular}{@{}l|lllll@{}}
		\textbf{Hostname} & \textbf{Devices} & \textbf{DPH} & \textbf{\firebog{}} & \textbf{\moab{}} & \textbf{StopAd}
		\\ \toprule
		webads.bandsintown.com	& \roku: Wild 	& \xmark  &   \xmark & \xmark &\xmark \\
		ads-e-darwin.hulustream.com 	& \roku: Wild 	& \xmark  &   \xmark & \xmark &\xmark \\
		track-us.adformnet.akadns.net	& Apple TV	& \xmark  &   \xmark & \xmark &\xmark \\
		disneyads0-a.akamaihd.net 	& Samsung	& \xmark  &   \xmark & \xmark &\xmark \\
		advertising.weather.com	& Samsung	& \xmark  &   \xmark & \xmark &\xmark \\
		tag.adaraanalytics.com	& Vizio	& \xmark  &   \xmark & \xmark &\xmark \\
		\hline
		p.ads.roku.com 										  & \roku 	& \xmark  &   \xmark & \xmark &\xmark \\
		ads.ewscloud.com 									 & \roku 	& \xmark  &   \xmark & \xmark &\xmark \\
		collector.vhx.tv 									  & \roku 	& \xmark  &   \xmark & \xmark &\xmark \\
		%attribution.report 									  & \roku 	& \xmark  &   \xmark & \xmark &\xmark  \\
		trackingrkx.com 									 & \roku & \xmark  &   \xmark & \xmark &\xmark  \\
		%us-east-1-ads.superawesome.tv 						  & \roku 	& \xmark  &   \xmark & \xmark &\xmark \\
		%adtag.primetime.adobe.com 							  & \roku 	& \xmark  &   \xmark & \xmark &\xmark  \\
		track.sr.roku.com 								      & \roku 	& \xmark  &   \xmark & \xmark &\xmark \\
		router.adstack.tv 									  & \roku 	& \xmark  &   \xmark & \xmark &\xmark \\
		%static.s3-us-west-1		
		%adplatform-[1].amazonaws.com 		  & \roku 	&\xmark  &   \xmark & \xmark &\xmark   \\
		metrics.claspws.tv 		  & \roku 	&\xmark  &   \xmark & \xmark &\xmark   \\
		\hline
		myhouseofads.firebaseio.com	  & \firetv & \xmark  &   \xmark & \xmark &\xmark \\
		% measurements.s3-external-1
		%kraken-[2].amazonaws.com 	  & \firetv & \xmark  &   \xmark & \xmark &\xmark  \\
		%kinstruments-[2].amazonaws.com  & \firetv & \xmark  &   \xmark & \xmark &\xmark\\
		%venezia-[2].amazonaws.com 	   & \firetv &\xmark  &   \xmark & \xmark &\xmark \\
		firebaseremoteconfig.googleapis.com 				   & \firetv & \xmark  &   \xmark & \xmark &\xmark\\
		mads.amazon.com 									  & \firetv & \xmark  &   \xmark & \xmark &\xmark\\
		ads.aimitv.com 										   & \firetv & \xmark  &   \xmark & \xmark &\xmark \\
		%ads.aimitv.com.s3.amazonaws.com 					   & \firetv & \xmark  &   \xmark & \xmark &\xmark \\
		analytics.mobitv.com 								   & \firetv & \xmark  &   \xmark & \xmark &\xmark \\
		ad-playlistserver.aws.syncbak.com 					   & \firetv & \xmark  &   \xmark & \xmark &\xmark \\
		events.brightline.tv 					   & \firetv & \xmark  &   \xmark & \xmark &\xmark \\
	\end{tabular}
	\caption{False negatives in filter lists}
	\label{tab:false_negatives}
\end{table*}
\end{comment}

%\begin{itemize}
	%\item Check some of these hostnames with Crunchbase or VirusTotal?
	%\item Provide a table or a plot with these hostnames.
	%\item Check if any PII go to these hostnames.
	%\item Check how often these hostnames are contacted in the user data.
	%\item If time permits: randomly select 10 apps that contact at least one of the suspicious hostnames. Run the apps and see if ads get through. Inspect traffic around the app and adjust filter lists accordingly.
%\end{itemize}




==> analysis_fpos.tex <==

\begin{table*}[t]
	\small
	\begin{tabularx}{\textwidth}{| l | X | c  c | c  c | c  c | c  c | c  c |}
		\cline{2-12}\multicolumn{1}{c|}{} & \makecell[c]{\textbf{Application}} & \multicolumn{2}{c|}{\textbf{No List}} & \multicolumn{2}{c|}{\textbf{\piholelists{}}} & \multicolumn{2}{c|}{\textbf{\firebog{}}} & \multicolumn{2}{c|}{\textbf{\moab{}}} & \multicolumn{2}{c|}{\textbf{\stopad{}}} \\
		\multicolumn{1}{c|}{} & & \makecell[c]{No \\Ads} & \makecell[c]{No \\ Breakage} & \makecell[c]{No \\Ads} & \makecell[c]{No \\ Breakage} & \makecell[c]{No \\Ads} & \makecell[c]{No \\ Breakage} & \makecell[c]{No \\Ads} & \makecell[c]{No \\ Breakage} & \makecell[c]{No \\Ads} & \makecell[c]{No \\ Breakage} \\
		\hline
		\parbox[t]{1mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{\roku{}}}}} & YouTube	& \xmark & \scalecheck & \xmark & \scalecheck & \xmark & \scalecheck	& \xmark & \scalecheck & \xmark & \scalecheck \\
		%\roku{} & YouTube	& \scalecheck	& \xmark & \scalecheck & \xmark & \scalecheck & \xmark	& \scalecheck & \xmark & \scalecheck & \xmark \\
		& CBS News Live & \xmark & \scalecheck & \scalecheck & \red{\textbf{\xmarkbold}} & \scalecheck  & \red{\xmarkbold} & \scalecheck & \red{\xmarkbold} & \scalecheck & \scalecheck \\
		& The Roku Channel & \xmark	& \scalecheck & \scalecheck & \scalecheck & \scalecheck & \red{\xmarkbold} & \scalecheck & \scalecheck & \xmark & \scalecheck \\
		& Sony Crackle & \xmark	& \scalecheck & \xmark & \scalecheck & \scalecheck  & \scalecheck & \xmark & \scalecheck & \xmark & \scalecheck  \\
		& Tubi & \scalecheck & \scalecheck & \scalecheck & \scalecheck & ---  & \red{\xmarkbold}	& \scalecheck & \scalecheck & \scalecheck & \scalecheck \\
		& Pluto TV & \xmark & \scalecheck & \xmark & \scalecheck & \xmark & \scalecheck & \xmark & \scalecheck & \xmark & \scalecheck \\
		& iFood.tv & \xmark & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck	& \scalecheck & \scalecheck & \xmark & \scalecheck  \\
		& WatchFreeComedyFlix & \xmark & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \xmark & \scalecheck & \xmark & \scalecheck \\
		& Live Past 100 Well & \scalecheck	& \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck  \\
		& SmartWoman & \xmark & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck   \\
		\hline
		\parbox[t]{1mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{\firetv{}}}}} &  Pluto TV & \xmark & \scalecheck & \xmark & \scalecheck & \xmark & \scalecheck & \xmark & \red{\xmark} & \xmark & \red{\xmarkbold}  \\
		%\firetv{} & Pluto TV & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \red{\textbf{M}} & \xmark & \red{\textbf{S}}  \\
		& iFood.tv & \xmark & \scalecheck & \scalecheck & \scalecheck & --- & \red{\xmarkbold}	& --- & \red{\xmarkbold} & \scalecheck & \scalecheck  \\
		& Tubi & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck \\
		& Downloader & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck \\
		& The CW for Fire TV & \xmark & \scalecheck & --- & \red{\xmarkbold}  & --- & \red{\xmarkbold}	& --- & \red{\xmarkbold} & \xmark & \scalecheck \\
		& FoxNow & \xmark & \red{\xmark} & --- & \red{\xmarkbold} & --- & \red{\xmarkbold} & \xmark & \scalecheck & \xmark & \scalecheck \\
		& Watch TNT & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck	& \scalecheck & \scalecheck & \scalecheck & \scalecheck \\
		& KCRA3 Sacramento News and Weather & \xmark & \red{\xmark} & \scalecheck & \scalecheck & --- & \red{\xmarkbold}	 & --- & \red{\xmarkbold} & \xmark & \red{\xmark} \\
		& Watch the Weather Channel & \xmark & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \xmark & \scalecheck & \scalecheck & \scalecheck \\
		& Jackpot Pokers by PokerStars & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck & \scalecheck	 & \scalecheck & \scalecheck & \scalecheck & \red{\xmark} \\
		\hline
	\end{tabularx}
	\caption{Effectiveness and false positives for each of the four lists in Table~\ref{tab:filter-lists} when employed during manual interaction with 10 \roku{} apps and 10 \firetv{} apps. For ``no ads'', a checkmark indicates that no ads popped up during the experiment, a cross indicates that some ad(s) popped up during the experiment, and a dash indicates that no data is available (when breakage prevents interaction with the app altogether). For ``no breakage'', a checkmark indicates that the app functioned correctly, a cross indicates minor breakage, and a bolded cross indicates severe breakage.}
	\label{tab:false-positives}
\end{table*}



\subsection{What is being blocked: mistakes}
In Sec.~\ref{sec:labelling-analysis}, we studied the extent to which each of the four filter lists covered the hostnames in the different ecosystems.
However, high coverage does not necessarily imply effectiveness.
For example, a filter list may block the main \ats{} hostname, but if the application contains a fallback mechanism in which it contacts a secondary \ats{} that is not covered by the list, the net outcome for the user is the same as with no list---an ad will be shown.
Additionally, filter lists may also contain rules that lead to app breakage.
We refer to such rules as false positives.
As such, a false positive for our purposes here may indeed be an \ats{} endpoint (that needs whitelisting for a an app to remain usable).
%\blue{[Is FP proper terminology? What if the rule blocks an \ats{}, but doing so causes app breakage? It is not really a false positives as it is an \ats{}, thus the filter list did its job correctly.]}.

%\blue{[Maybe we need to mention somewhere around here that we only focus on ads because it has a visual element as opposed to tracking.]}


%%
\descr{method.}
We study the effectiveness of, and presence of false positives in, the four filter lists in Table~\ref{tab:filter-lists} by manually interacting with 10 apps from the \roku{} and the \firetv{} platforms while observing for ads and app breakage.
We pick the 10 apps from the set of apps in our lab datasets described in Sec.~\ref{sec:popular-app-testing}: four apps from the top free apps of each platform, three apps present on both platforms, and an additional three randomly selected apps for each platform.
For each app, we perform a series of five experiments: one control experiment in which we do not deploy any filter lists, and an additional four experiments in which we deploy a single filter list from Table~\ref{tab:filter-lists} at a time (we set up a \pihole{} for this purpose).
During each experiment, we attempt to trigger ads by playing multiple videos and/or live TV channels and fast-forwarding through video content, and we make note of any ads shown and any app breakage.
\blue{We define three levels of breakage: (1) no breakage; (2) minor breakage for when the app's main content remains availble, but the application suffers from smaller issues such as UI glitches or ocassional freezes; and (3) severe breakage for when the main content becomes unavailable or the app fails to launch.}

%We first perform a control experiment in which we make note of any ads shown and any app breakage
%For each app, we first perform a control experiment in which we interact with the app without applying any filter lists.


\descr{False Positives.} (push false negative discussion to next point)
The results from our experiments are summarized in Table~\ref{tab:false-positives}.
%\firebog{}, which also had best coverage (see Sec.~\ref{sec:labelling-analysis}), is by far the most effective filter lists for the two platforms we study, indicating that there is some correlation between coverage and effectiveness.
For the two platforms we study, \firebog{} is by far the most effective filter list, and \stopad{} is the least effective filter list.
These two lists were also the lists with the best and worst coverage (see Sec.~\ref{sec:labelling-analysis}), respectively, indicating that there is some correlation between coverage and effectiveness.
On the contrary, while \moab{} had slightly better coverage than \piholelists{}, \piholelists{} actually outperforms \moab{} significantly in terms of effectiveness.
\blue{[How do we want to angle this? Could also choose to say that the tendency is less clear for \moab{} and \piholelists{}, but still somewhat present.]}
\firebog{}'s ability to block \emph{all} ads in the Sony Crackle Roku app was especially impressive as this app was extremely heavy on ads, and neither of the other lists managed to just reduce the number of ads.
\firebog{}'s effect was even reflected in Sony Crackle's UI: a video's timeline in this app is a dashed line, and a block of ads is shown at each gap, but with \firebog{} enabled, the timeline became a solid line.
%This also applies if the user fast-forwards to the end of a movie, effectively meaning they will have to sit through multiple blocks of 4 or 5 ads to watch the last few minutes of a movie.
We also observe that a few apps manage to successfully serve ads, nomatter what filter list is deployed.
Pluto TV is particularly interesting as this holds true for both the Roku as well as the Fire TV versions of that app.
\blue{[Mabe we can infer something from the hostnames it shares and/or has unique for each platform?]}
While \firebog{} is the most effective list, it is also the list that causes the most breakage.
For \roku{}, \firebog{} prevented the live news feed in the CBS News Live app from playing, caused movies on the Roku Channel to report that they were no longer available in the middle of playback, and prevented Tubi from launching.
\blue{[Maybe Hieu adds some examples from \firetv{} test here as well.]}
In contrast, \stopad{} provides a breakage-free experience on \roku{}, and only a single case of severe breakage on \firetv{}, but also only managed to block ads in a single Roku app and two \firetv{} apps during our experiments.


In summary, while some of the filter lists in our study are effective, the same lists unfortunately also incur a significant amount of app breakage and must therefore be combined with whitelists specifically currated for the individual user's selection of apps to remain as effective as possible while still ensuring that the functionality of each app is preserved.
\blue{[Can we say that we see opportunity for future research in this space? E.g. apply our tools/datasets to profile individual apps' sets of hostnames and use this to (automatically) check what hostnames are necessary for app functionality and which are not---and from this build something that (automatically) tailors a block list to the set of installed apps?]}

%To see if the filter lists contain any false positives that can lead to app breakage, we used the following procedure. First, for each ecosystem in our \synthdataset, we retrieved a list of hostnames that were contacted by only one app and were labeled as \ats by only one of the three filter lists. Next, we randomly select 10 apps that send at least 10 requests to such hostnames. We then manually interact with each app for 10 minutes while applying all three filter lists to the outgoing traffic. We utilize PiHole \blue{[ref]} to apply the filter lists for both \roku{} and \firetv{} to block packets destined to hosts that appear in the filter lists. \blue{[TODO: maybe more details on how PiHole/AntMonitor blocking works?]}. While interacting with each app, we note of any app breakage (\eg \blue{[add some examples of what is broken]}) and the time around which the breakage occurred.



%Ideas for FPs in user data: (1) look at the volume of data returned by hosts that appear in filter lists. If the volume is large, then it's a possible false positive (large video); (2) identify apps in the userdata based on hostnames they contact and then test them manually?
\begin{comment}
\begin{table*}[t]
	\small
	\begin{tabular}{@{}l|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}@{}}
		\hline
		\textbf{Application} & \textbf{Control} & \textbf{\piholelists{}} & \textbf{\firebog{}} & \textbf{\moab{}} & \textbf{\stopad{}}
		\\ \toprule
		YouTube	& x	& x &   x & x & x \\
		CBS News Live & x	& x &   x & x & x  \\
		The Roku Channel & x	& x &   x & x & x \\
		Sony Crackle & x	& x &   x & x & x  \\
		Tubi & x & x &   x & x & x  \\
		Pluto TV & x	& x &   x & x & x \\
		iFood.tv & x	& x &   x & x & x  \\
		WatchFreeComedyFlix & x	& x &   x & x & x  \\
		Live Past 100 Well & x	& x &   x & x & x  \\
		SmartWoman & x	& x &   x & x & x   \\
		\hline
		Pluto TV 	  & x& x &   x & x & x  \\
		iFood.tv   & x & x &   x & x & x \\
		Tubi 	   & x & x &   x & x & x \\
		Downloader  				   & x & x &   x & x & x\\
		The CW for Fire TV  									  & x & x &   x & x & x\\
		FoxNow 									   & x& x &   x & x & x \\
		Watch TNT  					   & x& x &   x & x & x \\
		KCRA3 Sacramento News and Weather 								   & x & x &   x & x & x \\
		Watch the Weather Channel  					   & x & x &   x & x & x \\
		Pokerds by Pokerstars  					   & x & x &   x & x & x
	\end{tabular}
	\caption{False positives test results. }
	\label{tab:false_positives}
\end{table*}
\end{comment}


\begin{comment}
\begin{table*}[t]
	\small
	\begin{tabularx}{\textwidth}{| l | X | c  c | c  c | c  c | c  c | c  c |}
		\hline
		\textbf{Platform} & \textbf{Application} & \multicolumn{2}{c|}{\textbf{Control}} & \multicolumn{2}{c|}{\textbf{\piholelists{}}} & \multicolumn{2}{c|}{\textbf{\firebog{}}} & \multicolumn{2}{c|}{\textbf{\moab{}}} & \multicolumn{2}{c|}{\textbf{\stopad{}}} \\
		& & Ads & Breakage & Ads & Breakage & Ads & Breakage & Ads & Breakage & Ads & Breakage \\
		\hline
		\roku{} & YouTube	& \scalecheck	& \xmark & \scalecheck & \xmark & \scalecheck & \xmark	& \scalecheck & \xmark & \scalecheck & \xmark \\
		& CBS News Live & \scalecheck	& \xmark & \xmark & \red{\textbf{S}} & \xmark  & \red{\textbf{S}} & \xmark & \red{\textbf{S}} & \xmark & \xmark \\
		& The Roku Channel & \scalecheck	& \xmark & \xmark & \xmark & \xmark & \red{\textbf{S}} & \xmark & \xmark & \scalecheck & \xmark \\
		& Sony Crackle & \scalecheck	& \xmark & \scalecheck & \xmark & \xmark  & \xmark	& \scalecheck & \xmark & \scalecheck & \xmark  \\
		& Tubi & \xmark & \xmark & \xmark & \xmark & ---  & \red{\textbf{S}}	& \xmark & \xmark & \xmark & \xmark \\
		& Pluto TV & \scalecheck & \xmark & \scalecheck & \xmark & \scalecheck & \xmark & \scalecheck & \xmark & \scalecheck & \xmark \\
		& iFood.tv & \scalecheck & \xmark & \xmark & \xmark & \xmark & \xmark	& \xmark & \xmark & \scalecheck & \xmark  \\
		& WatchFreeComedyFlix & \scalecheck & \xmark & \xmark & \xmark & \xmark & \xmark	& \scalecheck & \xmark & \scalecheck & \xmark \\
		& Live Past 100 Well & \xmark	& \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark  \\
		& SmartWoman & \scalecheck & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark   \\
		\hline
		\firetv{} & Pluto TV & \scalecheck & \xmark & \scalecheck & \xmark & \scalecheck & \xmark & \scalecheck & \red{\textbf{M}} & \scalecheck & \red{\textbf{S}}  \\
		& iFood.tv & \scalecheck & \xmark & \xmark & \xmark & --- & \red{\textbf{S}}	& --- & \red{\textbf{S}} & \xmark & \xmark  \\
		& Tubi & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
		& Downloader & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
		& The CW for Fire TV & \scalecheck & \xmark & --- & \red{\textbf{S}}  & --- & \red{\textbf{S}}	& --- & \red{\textbf{S}} & \scalecheck & \xmark \\
		& FoxNow & \scalecheck & \red{\textbf{M}} & --- & \red{\textbf{S}} & --- & \red{\textbf{S}} & \scalecheck & \xmark & \scalecheck & \xmark \\
		& Watch TNT & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark	& \xmark & \xmark & \xmark & \xmark \\
		& KCRA3 Sacramento News and Weather & \scalecheck & \red{\textbf{M}} & \xmark & \xmark & --- & \red{\textbf{S}}	& --- & \red{\textbf{S}} & \scalecheck & \red{\textbf{M}} \\
		& Watch the Weather Channel & \scalecheck & \xmark & \xmark & \xmark & \xmark & \xmark & \scalecheck & \xmark & \xmark & \xmark \\
		& Jackpot Pokers by PokerStars & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark	& \xmark & \xmark & \xmark & \red{\textbf{M}} \\
		\hline
	\end{tabularx}
	\caption{Effectiveness and false positives for each of the four lists in Table~\ref{tab:filter-lists} when employed during manual interaction with 10 \roku{} apps and 10 \firetv{} apps. For ads, a checkmark indicates that one or more ads popped up during the experiment, a cross indicates that no ads popped up during the experiment, and a dash indicates that no data is available (when breakage prevents interaction with the app altogether). For breakage, M indicates minor breakage, S indicates severe breakage, and a cross indicates that the app was working as intended. \blue{[TODO We need to discuss how we define breakage. If we just make it binary, the presentation in this table will be more readable. Defining levels of breakage may also be very subjective. E.g., for Roku CBS News, the live news won't play with \firebog{} enabled, but other content such as 60 Minutes will---is this severe breakage because the main news feed won't play, or is it only minor since other content in the app remains usable?]}}
	\label{tab:false-positives}
\end{table*}
\end{comment}
% minor for jackpot: app broke after a game, had to restart it
%


==> analysis_labelling.tex <==
In this section, we evaluate the effectiveness of well-known block lists in blocking advertisers and trackers in the smart TV ecosystem.
%
how would users would apply such lists
%
pi-hole or other conceptually similar solutions 
%
hosts-based lists that dns black holing for two reasons: 
%
1) unlike browser based URL lists (easylist and easyprivacy) that have access to url due to TLS
%
2) performance ?


%%
\descr{block list selection.}
We deliberately choose filter lists that only consider the hostname so as to evaluate readily available privacy-preserving tools that can be applied by non-technical users.
%
Specifically, as these lists can operate on encrypted traffic, they can be put to work by setting up a \pihole{} on any networked middle-box using the ``one-click'' installer provided by \pihole.
%
In contrast, more granular filter lists such as EasyList also consider the URL path and thus need access to plaintext traffic\footnote{The \firebog{} filter list contains modified versions of EasyList and EasyPrivacy designed to operate only on hostnames.}.
%
As shown in Sec.~\ref{sec:popular-app-testing}, most traffic on the \roku{} and \firetv{} platforms is encrypted \blue{[TODO verify after updating numbers.]}.
%
While traffic decryption is possible for \firetv{} using tools such as \cite{antmonitoross}, this does not generalize to the large set of other smart TV platforms present in the market.


%%
%%
Table~\ref{tab:filter-lists} lists in the realm of smart TVs by applying them to the traffic in the datasets from Sections~\ref{sec:in-the-wild} and~\ref{sec:popular-app-testing}.
%
We include the default \pihole{} block lists (\piholelists{}) to imitate the experience of a novice \pihole{} user, and the popular \firebog{} lists to imitate the experiences of more advanced users.
%
We also include Mother of All Ad-Blocking (\moab{}) \cite{moab} as it one of the most extensive lists with more than 255K rules \blue{[Could also argue that it enables us to compare the smart TV \ats{} ecosystem with the mobile \ats{} ecosystem if we find something useful for this list in the FN/FP analysis]}.
%
The selected lists cover network-wide and/or smart TV specific blocking from both the open source community (\pihole{}) as well as commercial solutions (\stopad{}).



\begin{table}[t!]
	\small
	\centering
	\begin{tabularx}{\columnwidth}{|X|X|r|}
		\hline
		\textbf{Filter list} & \textbf{Target platforms} & \# Rules \\
		\hline
		Mother of All Ad-Blocking (\moab{}) & Android & 255220 \\
		\hline
		Firebog advertising and tracking lists (\firebog{}) & Pi-Hole  & 162068 \\
		\hline
		Default Pi-Hole block lists (\piholelists) & Pi-Hole  & 133530 \\
		\hline
		StopAd & FireTV, Android TV, Android, Windows, macOS, iOS & 2745 \\
		\hline
	\end{tabularx}
	\caption{Four popular filter lists we used to match our datasets against.} % \blue{[Add links to lists?]}} %
	\label{tab:filter-lists} 
\end{table}




\descr{How much is being blocked?}


\begin{table}[t!]
	\small
	\centering
	\begin{tabularx}{\columnwidth}{|X|r|r|r|r|r|r|r|}
		\cline{3-7} \multicolumn{2}{c}{} & \multicolumn{5}{|c|}{\textbf{Blocked}} \\
		\hline
		\textbf{Dataset} & \textbf{Total} & \textbf{\piholelists{}} & \textbf{\firebog{}} & \textbf{\moab{}} & \textbf{\stopad{}} & \textbf{All lists} \\
		\hline
		\appleitw{} & 3179 & 10\% & \cellcolor{green} 13\% & 12\% & 5\% & 14\% \\
		\hline
		\samsungitw{} & 1765 & 14\% & \cellcolor{green} 19\% & 15\% & 8\% & 21\% \\
		\hline
		\chromecastitw{} & 1576 & 9\% & \cellcolor{green} 15\% & 15\% & 5\% & 16\% \\
		\hline
		\rokuitw{}: Wild & 2312 & 15\% & \cellcolor{green} 19\% & 18\% & 7\% & 22\% \\
		\hline
		\vizioitw{} & 942 & 16\% & \cellcolor{green} 18\% & 16\% & 11\% & 19\% \\
		\hline
		\lgitw{} & 627 & 45\% & \cellcolor{green} 54\% & 50\% & 27\% & 56\% \\
		\hline
		\sonyitw{} & 119 & 16\% & \cellcolor{green} 24\% & 16\% & 7\% & 25\% \\
		\specialrule{1.2pt}{0pt}{0pt}
		\roku{}: Testbed & 2191 & 17\% &  \cellcolor{green} 22\% & 20\% & 9\% & 25\% \\
		\hline
		%Lab & \roku{} & Flows & 102.4K & 39.3K (38\%) &  \cellcolor{green} 42.2K (41\%) & 40K (39\%) & 12.5K (12\%) \\ % raw numbers: Roku: flows & 102404 &  DPH 39306 (X\%) &   FAT 42157 (X\%) & MoAAB 39991 (X\%) & 12494 (X\%) \\
		%\hline
		\firetv{}: Testbed & 1734 & 22\% & \cellcolor{green} 27\% & 22\% & 9\% & 30\% \\
		\hline
		%Lab & \firetv{} & Flows & 228.6K & 46.7K (20\%) &  \cellcolor{green} 52.8K (23\%) & 44.6K (20\%) & 12.9K (6\%) \\ % raw numbers: FireTV: flows & 228557 & 46669 (X\%) &  52792 (X\%) & 44637 (X\%) & 12940 (X\%) \\
		%\hline
		
		% TODO: does it make sense to do flows per platform for In the Wild?
		%In the Wild & \appleitw{}: flows & x & x (x\%) & \cellcolor{green} x (x\%) & x (x\%) &x (x\%) \\
		
		
	\end{tabularx}
	\caption{ We match each dataset collected in the wild (Sec. .~\ref{sec:in-the-wild} - top rows) or in our testbed (Sec.~\ref{sec:popular-app-testing} - bottom rows) against eacg of the four filter lists and we show the coverage of hostnames. \firebog{}. turns out to have the highest coverage in each dataset.} % Potential false positives not considered.}
	\label{tab:filter-list-performance-summary}
\end{table}


Table~\ref{tab:filter-list-performance-summary} summarizes the four filter lists' \blue{coverage}, defined as the number of hits (not considering any potential false positives), on the \roku{} and \firetv{} datasets.
We show the \blue{coverage} both in terms of number of hostnames blocked as well as the number of flows blocked.
The results reported here were obtained using filter lists downloaded from their respective sources on \blue{2019-04-29}\footnote{\blue{StopAd was extracted from the Android APK on 2019-04-01. We could not retrieve an updated version on 2019-04-29 as the APK was made unavailable, possibly due to legal issues.}}.
All lists were converted to Adblock Plus syntax \cite{abpsyntax}, and matching was performed using \texttt{AdblockParser v0.7} \cite{adblockparser}. \blue{[Can drop explanation of how we perform matching to avoid questions about why we didn't just do simple string \texttt{contains()}.]}
As expected, the longer filter lists (\moab{} and \firebog{}) have best \blue{coverage}.
Despite being signficantly shorter, \firebog{} slightly outperforms \moab{}.
While \moab{} targets the mobile platform, \firebog{} includes lists specifically curated for smart TVs.
Thus this gives a first indication that the smart TV \ats{} ecosystems differ from other platforms' \ats{} ecosystems, similar to what was shown in \cite{shuba2018nomoads} in the case of the web vs. mobile platforms.
Interestingly, \stopad{}, which specifically targets smart TV platforms, is the list with the worst \blue{coverage}.
This may potentially be explained by the fact that its ruleset is two orders of magnitude smaller than the other three lists' rulesets, but also leaves the question of whether the other lists simply include a high number of false positives when applied to smart TV ecosystems.
We return to this in Sec.~\ref{sec:fpos-analysis} \blue{[Make sure we do :)]}.


\descr{Impact of app presence.}
We next perform a comparison of \emph{shared hostnames} vs. \emph{app-specific hostnames}.
A shared hostname is a hostname that is contacted by two or more apps from the same ecosystem, and an app-specific hostname is a hostname that is only contacted by a single app.
Our hypothesis is that hostnames pertaining to \ats{} are likely to be contacted by a large number of apps, as ATSs are usually provided by third-parties and hence shared across apps.
Our \roku{} dataset contains \blue{670} shared hostnames and \blue{1531} app-specific hostnames, while these numbers are \blue{Q} and \blue{Z} for \firetv{}.
For \roku{}, only \blue{X\%} of app-specific hostnames are blocked by \emph{any} of the four filter lists, whereas this number \blue{more than doubles to Y\%} for shared hostnames.
Similarly, these numbers are \blue{Q\%} and \blue{Z\%}, respectively, for \firetv{}.
As anticipated, shared hostnames are more likely to be \ats{}.
Figures~\ref{fig:roku-blocking-as-func-of-hostname-popularity} and \ref{fig:firetv-blocking-as-func-of-hostname-popularity} show how this tendency develops as hostname popularity (number of apps contacting a hostname) increases.
Although most pronounced in the case of Roku, for both ecosystems, we see that the likelihood that a hostname is \blue{(labeled as)} an \ats{} increases as hostname popularity increases until finally plateuing when a hostname is shared by 10 or more apps. \blue{[Say that this makes sense: one developer may have a couple of apps and use the same domain to deliver content to both of apps, but highly unlikely same developer has 10 apps?]}.
Currently, filter lists are manually currated.
Since shared hostnames are more likely to be \blue{(labeled as)} \ats{}, tools such as \rokutool{} and \firetvtool{} may be used to generate high quality filter list candidate rules as they can automatically discover shared hostnames by exercising thousands of apps.


\begin{figure}[t!]
	\centering
	\includegraphics[width=\columnwidth]{figures/roku-blocking-as-func-of-hostname-popularity.pdf}
	\caption{Roku: percentage of hostnames blocked as hostname popularity increases. (We refer to hostname "popularity'' as the rank defined by the number of apps that contact the hostname.). \textcolor{red}{AM:Merge with other figure (commented out) -+add main text describing them}}
	\label{fig:roku-blocking-as-func-of-hostname-popularity}
\end{figure}


\begin{figure}[t!]
	\centering
	\includegraphics[width=\columnwidth]{figures/firetv-blocking-as-func-of-hostname-popularity.pdf}
	\caption{FireTV: percentage of hostnames blocked / not blocked as hostname popularity increases. Numbers on the \textit{x}-axis indicate popularity. For example, if $x=4$, this means the set of hostnames such that all hostnames in that set are contacted by four or more apps.}
	\label{fig:firetv-blocking-as-func-of-hostname-popularity}
\end{figure}


\descr{Impact of app ranking.}
To evaluate the filter list performance (on flows) further by popularity, we rely on the implicit ranking from the Top Featured list shown in Table ~\ref{tab:firetv-app-ranking-blocked}. We see similar results that match prior work \cite{merzdovnik2017block}, where filter lists perform the best on the top 200 apps across the board. For \moab, \pihole, and \firebog, we see that the performance drops on average about 13\% when comparing top to bottom tier apps ([1,200] versus [800, 1K]), with \pihole displaying the most drastic drop to 6\%. Interestingly, the commercial filter list, \stopad, displays consistent blocking performance across all app rankings, but it does have the least amount of blocked flows. Although this could be explained by its lower rules count when compared to other lists, it is still unexpected as \stopad is marketed towards the \firetv{} and Android TV ecosystems.


\begin{table}[t!]
	\begin{tabular}{|l|r|r|r|r|}
		\hline
		\multicolumn{1}{|c|}{\firetv{}} & \multicolumn{4}{c|}{\% of Blocked Flows} \\
		\textbf{Rank Interval} & \multicolumn{1}{c}{\textbf{\piholelists{}}} & \multicolumn{1}{c}{\textbf{\firebog{}}} & \multicolumn{1}{c}{\textbf{\moab{}}} & \textbf{\stopad{}} \\
		\hline
		$[1, 200)$ &  29\% &  32\% &  25\% & 6\% \\
		$[200, 400$ & 21\% & 23\% &  19\% & 5\% \\
		$[400, 600)$ & 21\% &  24\% & 21\% &  6\% \\
		$[600, 800)$ & 16\% &  18\% &  16\% & 4\% \\
		$[800, 1K)$ & 6\% &  22\% & 18\% & 6\% \\
		\hline
	\end{tabular}
	\caption{\firetv{}: percentage of blocked flows by app ranking.}
	\label{tab:firetv-app-ranking-blocked}
\end{table}




\descr{PII in blocked traffic.}
We revisit \pii{} exposure to explore how well the four filter lists block them. Table~\ref{tab:pii-firetv-roku-filter-list} summaries blocking of requests that contain \pii{} for any of the filter lists. We immediately see a clear distinction between blocking coverage for Advertising ID on \roku{} (94\%) when compared to \firetv{} (20\%). On the other hand, we see that the filter lists only perform well when blocking Account Name in \firetv{} (95\%). In addition, the filter lists fail to block the majority of fingerprinting \pii{} such as Serial Number and Device ID on \firetv{} but do an excellent job with blocking Location \pii{}. As a result of low percentages for blocking \pii{}, we deduce that all four filter lists need improvement for better coverage on \smarttv{} platforms like \roku{} and \firetv{} Thus, we explore the extent of filter lists weaknesses in the next sections.


\begin{table}[t]
	\small
	\begin{tabular}{@{}l|ll@{}}
		\multicolumn{1}{c|}{} & \multicolumn{2}{c}{By Requests} \\
		\textbf{PII Exposure} & \textbf{Roku} & \textbf{FireTV}
		 \\ \toprule
		
		Advertising ID &  94\% &  20\%   \\ % 4561, 1934
		Serial Number & 46\% & 0.6\%  \\ %864, 76
		Device ID & --  & 7\%  \\ %0, 889
		Account Name & 25\% & 95\%  \\ %2, 52
		%Device Model & 87\% & 0\%  \\ % 2220, 0
		%OS Version & 31\% & 2\%  \\ %21079, 724
		MAC Addr & -- & 100\%  \\ %38
		Location & 100\% & 99\%   \\ %95, 235
		%\toprule
		%Any & 31\% & 9\%  \\  %21079, 3752
		\toprule
	\end{tabular}
	\caption{PII exposure being blocked by any Filter Lists within each platform}
	\label{tab:pii-firetv-roku-filter-list}
\end{table}




%\subsection{Coverage and Shared Hostnames}
%\label{sec:labelling-analysis}


\begin{comment}
One observation is that all lists perform better in terms of number of flows blocked rather than number of hostnames blocked.
Intuitively, this makes sense: the primary purpose of a smart TV is to deliver video (on demand), meaning ``legitimate'' content will be delivered throughout an extended period of time over a single, long-lived connection as opposed to multiple short-lived connections.
In contrast, consider ads that pop up occasionally during video playback.
Leaving a connection open to fetch an ad every $m$ minutes would put unnecessary strain on the server during the idle periods between ads.
Moreover, the connection establishment delay does not play a role as the ad can be fetched in the background during video playback.
Thus the number of flows to \ats{} endpoints is likely to exceed the number of flows to endpoints that deliver content, explaining why the filter lists do better in terms of number of flows blocked rather than number of hostnames blocked.

Another observation is that block rates are significantly larger for the Roku than Fire TV, suggesting that advertisement and tracking is less widespread on Fire TV \emph{or} that the \ats{} ecosystem contains platform-specific hostnames not yet mapped by the filter lists.\blue{[Note: might no longer be true if we exclude the IPs discussed next.]}
However, 44\% of all distinct hostnames in the Fire TV dataset are not real hostnames, but rather IPs in the 52.216.0.0/16 subnet.
These show up as hostnames in our dataset as they appear in the HTTP \texttt{Host} header field, which we rely on in order to determine hostname information (see Sec.~\ref{sect:todo}).
The subnet is an Amazon subnet, and \emph{all} flows to IPs in this subnet are used for the same purpose, namely to send an HTTP request for the file identified by the path \texttt{/kindle-wifi/wifistub.html}.
According to the Alexa documentation, these requests are sent by the Fire TV to test for Internet connectivity \cite{alexanetworkconnectivity}. \blue{[Move this discussion of these hostnames to Sec.~4; then we can exclude them from the filter list analysis and get more meaningful results.]}
%From manual inspection of the packet traces, we confirmed that the DNS resolution

\end{comment}

%\blue{[Get back to this.]}




%\subsubsection{Hostnames contacted by one or more Apps}

% \blue{[TODO get actual numbers for this section. Remove 52.216.0.0/16 subnet from firetv data to get cleaner results.]}






%Intuitively, this makes sense: the primary purpose of a smart TV is to stream video content, thus legitimate end-content is likely to be downloaded through a single long-lived connection as opposed to multiple short-lived connections in order to avoid the delay incurred when establishing a connection. In contrast, ads and tracking related reques

%Intuitively, this makes sense: the primary purpose of a smart TV is to serve video content, thus legitimate end-content will be downloaded and legitimate flows will therefore be long-lived. In contrast, ads and tracking




%\subsubsection{ Filter Lists on FireTV}
%\label{sec:labelling-analysis-firetv}




\begin{comment}
\begin{table*}
	\small
	\centering
	\begin{tabularx}{\textwidth}{|l|l|X|r|r|r|r|r|r|}
		\cline{5-9} \multicolumn{4}{c}{} & \multicolumn{5}{|c|}{\textbf{Blocked}} \\
		\hline
		\textbf{Dataset}& \textbf{Platform} & \textbf{Desc.} & \textbf{Total} & \textbf{\piholelists{}} & \textbf{\firebog{}} & \textbf{\moab{}} & \textbf{\stopad{}} & \textbf{Any} \\
		\hline
		In the Wild & \appleitw{} & Hostnames & 3179 & 10\% & \cellcolor{green} 13\% & 12\% & 5\% & 14\% \\
		\hline
		In the Wild & \samsungitw{} & Hostnames & 1765 & 14\% & \cellcolor{green} 19\% & 15\% & 8\% & 21\% \\
		\hline
		In the Wild & \chromecastitw{} & Hostnames & 1576 & 9\% & \cellcolor{green} 15\% & 15\% & 5\% & 16\% \\
		\hline
		In the Wild & \rokuitw{} & Hostnames & 2312 & 15\% & \cellcolor{green} 19\% & 18\% & 7\% & 22\% \\
		\hline
		In the Wild & \vizioitw{} & Hostnames & 942 & 16\% & \cellcolor{green} 18\% & 16\% & 11\% & 19\% \\
		\hline
		In the Wild & \lgitw{} & Hostnames & 627 & 45\% & \cellcolor{green} 54\% & 50\% & 27\% & 56\% \\
		\hline
		In the Wild & \sonyitw{} & Hostnames & 119 & 16\% & \cellcolor{green} 24\% & 16\% & 7\% & 25\% \\
		\hline
		Lab & \roku{} & Hostnames & 2191 & 17\% &  \cellcolor{green} 22\% & 20\% & 9\% & 25\% \\
		\hline
		%Lab & \roku{} & Flows & 102.4K & 39.3K (38\%) &  \cellcolor{green} 42.2K (41\%) & 40K (39\%) & 12.5K (12\%) \\ % raw numbers: Roku: flows & 102404 &  DPH 39306 (X\%) &   FAT 42157 (X\%) & MoAAB 39991 (X\%) & 12494 (X\%) \\
		%\hline
		Lab & \firetv{} & Hostnames & 1734 & 22\% & \cellcolor{green} 27\% & 22\% & 9\% & 30\% \\
		\hline
		%Lab & \firetv{} & Flows & 228.6K & 46.7K (20\%) &  \cellcolor{green} 52.8K (23\%) & 44.6K (20\%) & 12.9K (6\%) \\ % raw numbers: FireTV: flows & 228557 & 46669 (X\%) &  52792 (X\%) & 44637 (X\%) & 12940 (X\%) \\
		%\hline
		
		% TODO: does it make sense to do flows per platform for In the Wild?
		%In the Wild & \appleitw{}: flows & x & x (x\%) & \cellcolor{green} x (x\%) & x (x\%) &x (x\%) \\
		
		
	\end{tabularx}
	\caption{The four filter lists' coverage on the datasets from Sections~\ref{sec:in-the-wild} and \ref{sec:popular-app-testing}. List with highest coverage highlighted in each row. Potential false positives not considered.}
	\label{tab:filter-list-performance-summary}
\end{table*}
\end{comment}



%\subsection{Shared Hostnames}
%\blue{Not sure if we want to move this to sect. 4.}

%\begin{figure}[h]
%	\centering
%	\includegraphics[width=\columnwidth]{figures/roku-filter-lists-relative-performance-hostnames.pdf}
%	\caption{Percentage of the set of distinct hostnames in the Roku dataset that were blocked by the considered filter lists.}
%	\label{fig:roku-filter-lists-relative-performance-hostnames}
%\end{figure}

%\begin{figure}[h]
%	\centering
%	\includegraphics[width=\columnwidth]{figures/roku-filter-lists-relative-performance-requests.pdf}
%	\caption{Percentage of the requests (defined as reassembled HTTP or TLS handshakes with SNI) in the Roku dataset that were blocked by the considered filter lists.}
%	\label{fig:roku-filter-lists-relative-performance-requests}
%\end{figure}

%\begin{figure}[h]
%	\centering
%	\includegraphics[width=\columnwidth]{figures/firetv-filter-lists-relative-performance-hostnames.pdf}
%	\caption{Percentage of the set of distinct hostnames in the FireTV dataset that were blocked by the considered filter lists.}
%	\label{fig:firetv-filter-lists-relative-performance-hostnames}
%\end{figure}

%\begin{figure}[h]
%	\centering
%	\includegraphics[width=\columnwidth]{figures/firetv-filter-lists-relative-performance-requests.pdf}
%	\caption{Percentage of the requests (defined as reassembled HTTP or TLS handshakes with SNI) in the FireTV dataset that were blocked by the considered filter lists. \blue{Emty hostnames and local IPs in the 10.0.1.0/24 range not considered.}}
%	\label{fig:roku-filter-lists-relative-performance-requests}
%\end{figure}



%We deliberately focus on filter lists that only consider the hostname rather than more granular filter lists such as EasyList, which also consider the URL path and therefore need access to decrypted traffic.
%Although traffic decryption is possible for \firetv{} using tools such as \cite{antmonitoross}, this does not generalize to the large set of other smart TV platforms.



%We study the Roku and FireTV platforms' \ats{} ecosystems by matching the collected, filtered traffic against four filter lists (see Table~\ref{tab:filter-lists}).
%With the chosen filter lists, we cover the current state of the art in terms of network-wide and/or smart TV specific blocking from both the open source community (Pi-Hole) as well as commercial solutions (StopAd).
%We include the default Pi-Hole block lists to imitate the experience of a novice Pi-Hole user, and the popular Firebog lists to imitate the experiences of more advanced users.
%We also include Mother of All Ad-Blocking (\moab{}) as it one of the most extensive lists with more than 255K rules \blue{[Could also argue that it enables us to compare the smart TV \ats{} ecosystem with the mobile \ats{} ecosystem if we find something useful for this list in the FN/FP analysis]}.

%The four filter lists are essentially analogous to a \texttt{hosts} file in that they only consider the hostname when determining if a connection should be blocked.
%In contrast, filter lists such as EasyList \blue{[add-ref]} and EasyPrivacy \blue{[add-ref]} are more fine-grained as they also take the path section of a URL  and HTTP headers into consideration\footnote{The Firebog Advertising and Tracking lists contain modified versions of EasyList and EasyPrivacy designed to work like a \texttt{hosts} file.}.
%These lists can hence block on a per request basis instead of blocking an entire connection, but need to operate on plaintext HTTP (they are usually used by browser plugins which intercept HTTP requests before encryption, if any, is applied).
%Since the Roku's traffic is captured on a middlebox\footnote{With no option for platform-wide MITM decryption as installation of custom certificates is done on a per channel basis as part of each channel's application code.}, we only have access to the ciphertext for flows that use encryption.
%We therefore purposefully exclude granular filter lists such as EasyList from our comparison as such lists would operate under a severe handicap (the URL's path and the HTTP headers are not available for encrypted flows).

%Matching was performed using \texttt{AdblockParser v0.7} \cite{adblockparser}, a Python package that matches HTTP(S) requests against filter rules written in Adblock Plus syntax \cite{abpsyntax}. 

==> analysis_pii.tex <==

%\subsubsection{PII and Filter Lists}
%\label{sec:piis-list-analysis}



